Neural Theorem Proving for Verification Conditions: A Real-World Benchmark

Theorem proving is fundamental to program verification, where the automated proof of Verification Conditions (VCs) remains a primary bottleneck. Real-world program verification frequently encounters hard VCs that existing Automated Theorem Provers (ATPs) cannot prove, leading to a critical need for extensive manual proofs that burden practical application. While Neural Theorem Proving (NTP) has achieved significant success in mathematical competitions, demonstrating the potential of machine learning approaches to formal reasoning, its application to program verification--particularly VC proving--remains largely unexplored. Despite existing work on annotation synthesis and verification-related theorem proving, no benchmark has specifically targeted this fundamental bottleneck: automated VC proving. This work introduces Neural Theorem Proving for Verification Conditions (NTP4VC), presenting the first real-world multi-language benchmark for this task. From real-world projects such as Linux and Contiki-OS kernel, our benchmark leverages industrial pipelines (Why3 and Frama-C) to generate semantically equivalent test cases across formal languages of Isabelle, Lean, and Rocq. We evaluate large language models (LLMs), both general-purpose and those fine-tuned for theorem proving, on NTP4VC. Results indicate that although LLMs show promise in VC proving, significant challenges remain for program verification, highlighting a large gap and opportunity for future research.

==> iclr2026/sections/intro.tex <==
\section{Introduction}\label{sec:intro}
% Yes, we need the table but maybe in related works or somewhere in the introduction
%\joshcommand{on the intro, I would create a figure like the table1: https://arxiv.org/pdf/2505.10610}

% Introduce Neural Theorem Proving, existing achievements, mainly in mathematical competitions.
% TODO: add explanation to interactive theorem provers

Neural Theorem Proving (NTP) leverages Large Language Models to generate formal proofs in mechanizedtheorem proving languages, enabling automated verification of mathematical judgments through machine learning~\citep{minervini2018towards}.
Recent successes in Neural Theorem Proving (NTP)~\citep{DeepSeekProver,GoedelProver,....}, especially the silver medal performance at the International Mathematical Olympiad~\citep{AlphaProver,SeedProver}, have shown that LLMs possess a certain degree of formal reasoning capability.

While existing NTP research primarily focuses on mathematical judgments, the judgments studied in theorem proving are not restricted to mathematical statements but also extend to program properties~\citep{HARRISON2014135}.
In fact, this forms the foundation of program verification --- program properties are expressed as judgments to be proven by theorem proving.

Although NTP for mathematical competitions has yet to demonstrate real-world value, program verification is a field that is widely deployed and critically needed by industry~\citep{AWSFormal,DARPA-HACMS,NASA-CR}.
Typical examples include cyber security~\citep{NCSC}, aerospace~\citep{ECSS,RTCA}, and healthcare~\citep{FDA}.

%The UK National Cyber Security Centre highlights program verification for critical system security~\citep{NCSC}; the European Space Agency’s ECSS-Q-ST-80C recognizes program verification as a means to meet rigorous software assurance in space systems~\citep{ECSS}; RTCA DO-333 accepts program verification as certification evidence in aerospace~\citep{RTCA}.
%and FDA guidance endorses such verification in medical device compliance~\citep{FDA}.

%Program verification delivers real-world value by providing rigorous assurance of software correctness, reducing costly defects, and strengthening safety and security.
%Pogram verification has direct impact on ensuring the cyber safety of human daily life, preventing software defects that cost US companies upwards of \$2.08 trillion How much could software errors be costing your company? · Raygun Blog annually

%While celebrating this victory, perhaps it is time to examine the value that NTP has actually brought to industry and academia.
%Initially, NTP was expected to offer a method for improving the mathematical reasoning capability of LLMs~\citep{citation}. However, NTP has not yet been adopted by mainstream general LLMs to improve their mathematical reasoning capabilities.
%In academic fields, one potential value lies in formalized mathematics --- automatically verifying the correctness of mathematical proofs.
%Despite pioneering efforts~\citep{APE}, the major NTP research works remain focused on competitions~\cite{SeedProver,more}, leaving a substantial gap with real-world mathematical research.

%One value is that Neural Theorem Proving is expected to be able to improve the general reasoning capability of LLMs. However, despite of suggestive studies, the direct conclusive evidences to support this are still insufficient. (Need references to support). Though SeedProver won the IMO silver medal this year, formal language modelsa still fail to beat down the informal language models like Gemini pro etc which won the gold medal this year.
% Second,

% Introduce the other application of theorem proving

% Nonetheless, formalized mathematics is not the only application of theorem proving.
% What actually occupies a dominant position in mainstream research is \emph{program verification}, as evidenced by trends in major conferences where ITP is used (??\% for formalized mathematics, ??\% for program verification, in the recent POPL, PLDI, ITP, LICS, and CAV).

% The impact of program verification

% ### In the next few paragraphs, we show: Theorem proving resides at the heart of program verification's main bottleneck.

Despite this strong industry demand, adoption of program verification remains concentrated in specific safety-critical domains rather than achieving widespread use~\citep{Tyler2023,Gleirscher2023}.
%Although the field has been studied for more than half a century~\citep{HoareTriple} and numerous industrial verifiers have been developed and deployed~\citep{Dafny,VCC,Verus}, adoption remains concentrated in specific safety-critical domains rather than achieving widespread use~\citep{Tyler2023,Gleirscher2023}.
A major impediment is the heavy demand for substantial manual effort from specialized experts~\citep{DARPA2025FormalMethodsPortfolio,AWS-Complain}.
Among these manual efforts, a central problem is the proving of \emph{Verification Conditions (VCs)}~\citep{Boogie}.
%
\begin{definition}
Given a program and a property, a \emph{Verification Condition (VC)} is a mathematical proposition that, when proven true, guarantees the program satisfies the desired property.
\end{definition}

% \input{iclr2026/figures/VCG}
% As illustrated in \cref{fig:verification}, the standard program verification workflow~\citep{VCC,Dafny,Boogie} centers on generating and proving VCs, and VCs are the direct theorem-proving targets.

Conventionally, VC proofs are carried out by Automated Theorem Provers (ATPs), which excel only at a limited domain of VCs, and require human intervention when automatic proof attempts fail or time out.
Taking the widely-used industry tool Frama-C~\citep{FramaC} as an example, a linked list library requires $\sim$800 lines of manual annotations for helping VC proofs, nearly matching lines of the original C code.
This heavy reliance on manual intervention makes automated proving of VCs a major bottleneck in program verification.

Given the central role of VCs in program verification and the limitations of current ATPs, we explore whether NTP could offer a more effective approach to automated VC proving.
To investigate this possibility, we define the task of Neural Theorem Proving for Verification Conditions (NTP4VC):
\begin{definition}
The task of \emph{Neural Theorem Proving for Verification Conditions (NTP4VC)} aims to apply the machine learning techniques adopted in NTP to conduct the formal proving of VCs.
\end{definition}

To advance its development, we present the first benchmark for this task, also named \emph{NTP4VC}.
As illustrated in \cref{fig:pipeline}, this benchmark consists of VCs that are extracted using the industrial verification pipeline Why3~\citep{Why3} and Frama-C~\citep{FramaC}, from both minimal programs covering challenging algorithms and data structures, and real-world C verification projects that involve the Linux kernel's scheduler and Contiki OS's memory allocator and linked-list library.

\input{iclr2026/figures/pipeline}


% While existing NTP works~\citep{FVEL,Rango} have explored verification-related theorem proving, much of their work focuses on proving auxiliary lemmas used by program verifiers and models --- such as those for preliminaries (e.g., arithmetic of bounded integers), programming language models (e.g., memory operation effects), and abstract program models (e.g., properties of the binary tree algebra) --- rather than VCs.
% For example, no VC is involved in the 1000 test cases by \citet{FVEL}.
% The gap between auxiliary lemmas and actual VCs is crucial because VCs are the proof goals that arise directly from program verification workflows.
% Although benchmarks constructed from auxiliary lemmas may assess models' knowledge in verification-related theories and abstract program models, they cannot directly evaluate models' performance on the theorem-proving demands of program verification tasks.

Additionally, prior verification-related benchmarks are monolingual, and current NTP models are each trained for a single language, creating fragmentation where NTP development on verification-related tasks is isolated across formal languages. For example, the PALM model~\citep{PALM} trained for Rocq cannot be compared with Deepseek-Prover~\citep{Deepseek-Prover} trained for Lean on verification tasks. To address this fragmentation, we contribute a multilingual benchmark supporting Lean, Isabelle, and Rocq. We achieve this through a novel extraction pipeline that employs expert-written translation rules to automatically convert Why3 VCs into target languages, ensuring semantic equivalence and fair comparison across different ITP systems.


\clearpage

% Background: what is VC


%VC plays an even more important role in the theorem proving for program verification, because it is the direct theorem-proving target that a prover for program verification must handle.

%Given the source code of the target program and the specification of its desired behavior, an ideal program verifier is expected to decide whether the actual behavior of the program \emph{always} satisfies the specification. If so, the program is certified against the specification. However, 
%

Among these two components, while VCG has achieved (more or less) mature automation with substantial capabilities~\citep{SMTscales}, automated proving of VCs remains \emph{a major bottleneck} of automated program verification~\citep{VCproofHard,VCproofHard2,VCproofHard3,VCproofHard4,VCproofHard5}.
VC proofs are typically carried out by Automated Theorem Provers (ATPs), which excel only at specific domains of problems, and require human intervention when automatic proof attempts fail or time out (e.g., manual proofs and annotations for simplifying the generated VCs).
%VC proofs initially rely on manual verification using ITP.
%Some early work~\citep{seL4} requires 20x as many lines of manually written proof code as lines of source C code.
%Recently, VC proofs have shifted toward automated approaches using Automated Theorem Provers (ATPs) such as Satisfiability Modulo Theories (SMT) solvers~\citep{BSST21,SMT}.
% Challenges of current ATP
Taking the widely-used industry tool Frama-C~\citep{FramaC} as an example, a linked list library requires $\sim$800 lines of annotations, nearly matching lines of the original C code, due to the insufficient capability of existing ATPs.
%About 80\% of these annotations are due to the insufficient capability of existing ATPs.

% NTP is the key
%These heavy labor cost that are forced to mitigate the insufficient capability of existing ATPs, is one key factor that 严重 limits the wider application of program verification in the industry.

Given this demand for powerful VC provers, we consider whether NTP techniques could be applied to automated VC proving. This consideration is motivated by NTP's demonstrated success in competition-level mathematical proofs and the observation that both tasks involve formal reasoning over mathematical propositions.
While VCs arise from program verification workflows and competition problems are (in contrast) handcrafted mathematical puzzles, they share the fundamental requirement of constructing formal proofs within logical frameworks.
Although the specific proof strategies and domain knowledge may differ between these contexts, this common need for formal proof construction means that general NTP techniques can and should be evaluated on their success in VC proving, not just competition mathematics.
To enable such investigation, we define the task of Neural Theorem Proving for Verification Conditions (NTP4VC):
\begin{definition}
The task of \emph{Neural Theorem Proving for Verification Conditions (NTP4VC)} aims to apply the machine learning techniques adopted in NTP to conduct the formal proving of VCs.
\end{definition}



While existing NTP works~\citep{FVEL,Rango} have explored verification-related theorem proving, much of their work focuses on proving auxiliary lemmas used by program verifiers and models --- such as those for preliminaries (e.g., arithmetic of bounded integers), programming language models (e.g., memory operation effects), and abstract program models (e.g., properties of the binary tree algebra) --- rather than VCs.
For example, no VC is involved in the 1000 test cases by \citet{FVEL}.
The gap between auxiliary lemmas and actual VCs is crucial because VCs are the proof goals that arise directly from program verification workflows.
Although benchmarks constructed from auxiliary lemmas may assess models' knowledge in verification-related theories and abstract program models, they cannot directly evaluate models' performance on the theorem-proving demands of program verification tasks.

% Motivation: Fragmented World.

% 定义了一个问题，发现没有有效的衡量 benchmark，因为各自是被割裂的，被 bound to 各自的语言，这导致不同语言上的选手无法相互竞争。可比较.

% 2. the capability of cross-language generation

% NTP bound to ITP language
% 之后所有的研究，只能跟自己相同语言圈子的比较，不能跟其他比较，这是个限制
% 对 NTP4VC community, 允许不同语言上的 NTP 去互相竞争（一个 benchmakr 的目的就是去让人竞争）
% VC 的问题本事是不受制于语言的，允许人们去衡量不同系统的优劣，选择不同的系统，

% Introduce the benchmark

Given the absence of a benchmark specifically for VC proving, we present the first benchmark for this task, also named \emph{NTP4VC}.
As illustrated in \cref{fig:pipeline}, this benchmark consists of VCs that are extracted using the industrial verification pipeline Why3~\citep{Why3} and Frama-C~\citep{FramaC}, from both minimal programs covering challenging algorithms and data structures, and real-world C verification projects that involve the Linux kernel's scheduler and Contiki OS's memory allocator and linked-list library.

Additionally, prior verification-related benchmarks are monolingual, with each benchmark limited to evaluating NTP models using one specific formal language.
Since current NTP models are each also trained for a single language, this creates a fragmentation where NTP development is isolated across formal languages.
For example, the PALM model~\citep{PALM} trained for Rocq cannot be compared with the Deepseek-Prover model~\citep{Deepseek-Prover} trained for Lean on verification tasks.
Addressing this fragmentation requires either multilingual models or multilingual benchmarks.
This work contributes to the latter --- our benchmark is multilingual, supporting Lean, Isabelle, and Rocq.
We achieve this through our novel extraction pipeline, which employs a translator to automatically convert Why3 VCs into the target languages.
Unlike LLM-based translation approaches that suffer from LLMs' unreliability, our translator is based on expert-written translation rules for each of the three target languages, explicitly chosen to ensure semantic equivalence across different ITP targets, ensuring fair comparison.



%However, we must clarify that our benchmark is not the first one for VCs.
%Previously, various benchmarks existed separately for different ITPs, making them incomparable and thereby fragmenting the research field --- preventing NTP systems built on different platforms from being compared with one another.
%A key feature of our benchmark is that it provides \emph{cross-prover} translations of identical VCs across mainstream ITPs, as illustrated in \cref{fig:pipeline}. Moreover, the sources of the translation are from two real-world industrial VCGs, Why3~\citep{Why3} and Frama-C~\citep{FramaC}.

%Move this somwhere else
%The VC language of Why3 falls within a small Higher-Order Logic that serves as a common foundation subsumed by all mainstream ITPs\footnote{including Isabelle~\citep{Isabelle}, Lean~\citep{Lean4}, Rocq~\citep{CoquandHuet1988CoC}, HOL4~\citep{SlindNorrish2008HOL4}, HOL Light~\citep{Harrison1996HLight}, Metamath~\citep{MegillWheeler2019Metamath}, F*~\citep{SwamyEtAl2011FStar}, Agda~\citep{Norell2009Agda}, and NuPRL~\citep{ConstableEtAl1986Nuprl}}, providing a degree of \emph{fairness} in comparing NTP systems built on different ITPs.

%All squares are existing industrial tools. The translation is based on language transformation rules that are carefully written by our experts in theorem proving and program verification, to ensure the semantic preservation of the translation.
%Thanking this carefully written translation, the benchmark cases in Isabelle, Rocq, and Lean share the same semantics of an identical VC source, thereby guaranteeing semantic equivalence among the interactive provers and rendering the benchmark \emph{fairly cross-prover}.

%to both cover as many program verification pain points as possible and include real verification cases from real-world engineering projects:
%The program verification cases included in this benchmark consist of two partitions:

At the end of the introduction, we summarize the paper's contributions.
\begin{enumerate}
\item We define the task of NTP4VC (\cref{sec:intro}), which aims to attack the automated proving of VC, a key bottleneck in program verification.
\item We propose a \emph{reliably automatic} method for extracting corpora from real-world verification projects. The implementation is open-sourced (\cref{sec:method}).
\item We present the first \emph{real-world} and \emph{multi-lingual} benchmark for the task of NTP4VC (\cref{sec:benchmark}).
%\item We evaluate leading NTPs and reasoning LLMs over the benchmark.
%As a surprising finding, we demonstrate for the first time that NTP can outperform a real industrial ATP solution for program verification --- Why3's strongest predefined hybrid ATP strategy that combines Z3~\citep{Z3}, CVC5~\citep{CVC5}, Alt-Ergo~\citep{AltErgo}, and SPASS~\citep{SPASS}.
\end{enumerate}


% VC 是直接的 the target proof obligation of program verification
% others are auxiliary


==> iclr2026/tables/pearl_category.tex <==
\begin{wraptable}{r}{5.3cm}
\centering
\setlength{\tabcolsep}{4pt}
\caption{Categories of the benchmark}\label{tab:categories}
\vspace*{-2em}
\begin{tabular}{lcc}\\\toprule  
Category & \!\!Number & ATP pass \\\midrule
\multicolumn{3}{l}{\it pearls of programs}\\[.2em]
Algorithm       & 62 & 19.35\%\\[.1em]
Data Structure\!\!\! & 83 & 20.48\%\\[.1em]
Calculation     & 74 & 20.27\%\\[.1em]
Engineering     & 65 & 20.00\%\\[.1em]
Competition     & 52 & 19.23\%\\[.2em]
\multicolumn{3}{l}{\it real C verification}\\[.2em]
Function        & 87 & 16.09\%\\[.1em]
Loop            & 110 & 18.18\%\\[.1em]
Memory          &  70 & 21.43\%\\[.1em]
Invalid Arg.    &  69 & 20.29\%\\\midrule
Total           & 672 & 19.35\% \\
\bottomrule
\end{tabular}
\vspace*{-5em}
\end{wraptable} 

